Graph-based Joint Signal / Power Restoration for Energy Harvesting Wireless Sensor Networks

The design of energy and spectrally efficient Wireless Sensor Networks (WSN) is crucial to support the upcoming expansion of IoT/M2M mobile data traffic. In this work, we consider an energy harvesting WSN where sensor data are periodically reported to a Fusion Center (FC) by a sparse set of active sensors. Unlike most existing works, the transmit power levels of each sensor are assumed to be unknown at the FC in this distributed setting. We address the inverse problem of joint signal / power restoration at the FC- a challenging under-determined separation problem. To regularize the ill-posed problem, we assume both a graph-signal smoothness prior (signal is smooth with respect to a graph modeling spatial correlation among sensors) and a sparsity power prior for the two unknown variables. We design an efficient algorithm by alternately fixing one variable and solving for the other until convergence. Specifically, when the signal is fixed, we solve for the power vector using Simplex pivoting in linear programming (LP) to iteratively identify sparse feasible solutions, locally minimizing an objective. Simulation results show that our proposal can achieve very low reconstruction errors and outperform conventional schemes under reasonable assumptions

==> formulate.tex <==

The objective of our method is to optimize the energy/power allocation vector $\bm{\eta}$ and the reconstructed signal $\mathbf{\hat{x}}$ such that the reconstruction error is minimized. Hence, the considered optimization problem can be formulated as a trade-off between the reconstruction error and the signal smoothness prior with parameter $\lambda$ assuming a graph Laplacian matrix $L$, i.e., 
\begin{eqnarray}
   &  \underset{\bm{\eta},\mathbf{x}}{\mathrm{min}} \ J(\bm{\eta},\mathbf{x})=||\mathbf{y}-\Phi H \mathrm{diag}(\bm{\eta}) \mathbf{x}||_2^2+\lambda \mathbf{x}^TL\mathbf{x} \nonumber\\
   & \text{s.t.} \quad \mathbf{0} \leq \bm{\eta} \leq \bm{\eta}_{\mathrm{max}},    
\label{eq:opt}
\end{eqnarray}
where the constraints are on individual maximum energy constraints $\bm{\eta}_{\mathrm{max}}=[\bm{\eta}_{\mathrm{max},1}, \cdots, \bm{\eta}_{\mathrm{max},N}]^T$ and their non-negativity. 
%where $||\mathbf{x}||_2 = \sqrt{\sum_{j=1}^{n} |x_j|^2}$, $\lambda$ is parameter that makes a trade off between fidelity term and representation error, $\mu$ is the parameter of weight allocation, and $\mathbf{w}$ is the vector of weight allocated to each node. 

This is a non-convex optimization problem over two variables $\bm{\eta},\mathbf{x}$, making it difficult to solve.
Therefore, we propose an iterative search method which alternates between the optimizations of each variable, keeping the other one fixed. 
The details are as follows.

In Step 1, we initialize by setting, e.g., $\bm{\eta}=\bm{\eta}_{\mathrm{max}}$, and solve for $\mathbf{x}$ with fixed $\bm{\eta}$. By deriving the partial derivative of $J$ w.r.t. $\mathbf{x}$ and solving for $\frac{\partial J}{\partial \mathbf{x}}=0$, the estimate $\mathbf{\hat{x}}_i$ for iteration $i$ is determined as
\begin{eqnarray}
\mathbf{\hat{x}}_i & =& \left\{(\Phi H \mathrm{diag}(\bm{\hat{\eta}}_{i-1}))^H (\Phi H \mathrm{diag}(\bm{\hat{\eta}}_{i-1}))+\lambda L\right\}^{\dagger} \nonumber\\
&& \times (\Phi H \mathrm{diag}(\bm{\hat{\eta}}_{i-1}))^H \mathbf{y},
%	\mathbf{\hat{x}}_1=\left\{(\Phi H )^H (\Phi H )+\lambda L\right\}^{\dagger} (\Phi H )^{H} \mathbf{y},
\end{eqnarray}
where $\bm{\hat{\eta}}_{i-1}$ is the estimate of  $\bm{\eta}$ at the previous iteration ($\bm{\hat{\eta}}_{i-1}=\bm{\eta}_{\mathrm{max}}$ for $i=1$)  and $\dagger$ stands for pseudo-inverse operation. 

In Step 2, we first solve for $\bm{\eta}$ by fixing $\mathbf{x}$ to its estimate determined in the previous step, namely $\mathbf{x}=\mathbf{\hat{x}}_{i}$. Since the smoothness prior is independent of $\bm{\eta}$, and observing that $ \mathrm{diag}(\bm{\eta}) \mathbf{x}=\mathrm{diag}(\mathbf{x}) \bm{\eta}$, (\ref{eq:opt}) can be rewritten as 
\begin{eqnarray}
   &  \underset{\bm{\eta}}{\mathrm{min}} \ J({\bm{\eta}})=||\mathbf{y}-\Phi H \mathrm{diag}(\mathbf{\hat{x}}_{i}) \bm{\eta}||_2^2 \nonumber\\
   & \text{s.t.} \quad \mathbf{0} \leq \bm{\eta} \leq \bm{\eta}_{\mathrm{max}},    
\label{eq:opt_eta}
\end{eqnarray}
which is a convex optimization problem with boundary constraints on $\bm{\eta}$. Thus, the estimate $\bm{\hat{\eta}}_{i}$ can be determined numerically by standard convex optimization algorithms with linear constraints. Note that since $\Phi H \mathrm{diag}(\mathbf{\hat{x}}_{i})$ is a fat $M \times N$ matrix of rank $M$, i.e., there are more variables than observations, in general there will be an infinity of feasible solutions $\bm{\hat{\eta}}_{i}$. Thus, the core idea of our proposed method is to select the solution $\bm{\hat{\eta}}_{i}$ among all feasible ones that enables to activate the $M$ most connected sensor nodes $S_n$. This corresponds to sampling the $M$ sensor signals $x_n$ that provide the best representation of the global signal $\mathbf{x}$.
Our proposed sampling algorithm based on [Antonio] works as follows.




%Banphatree
%Consider term that having variable $\mathbf{x}$
%\begin{multline}
%||\mathbf{y-\Phi H Px}||_2^{2}
%+\lambda \mathbf{x^TLx}\\=
%\mathbf{(y-\Phi H P  x)^H(y-\Phi H P x)}+
%\lambda\mathbf{x^HLx}\\
%=\mathbf{y^Hy -2y^H\Phi H P x + x^H P^H H^H \Phi^H\Phi H P x+\lambda x^HLx }
%\end{multline}
%%--------------------------------------------------------------------
% Next in Step 2, fix $X$ to find $p$ when $p$ is a vector in $(\mathbb{R^{+}}\cup \{0\})^{N}$
%Define $\mathbf{X}$ is diagonal($\mathbf{x}$) matrix
%and $\mathbf{p}$ is vector that contain diagnal entry of matrix $\mathbf{P}$ .
%
%Consider term that having variable $\mathbf{p}$
%
%\begin{multline}
%||\mathbf{y-\Phi H X p}||_2^{2}
%+ \mu \textbf{p}^Tw\\=
%\mathbf{(y-\Phi H X p)^H(y-\Phi H X p)}+
%+ \mu \textbf{p}^Tw\\
%=\mathbf{y^Hy -2y^H\Phi H Xp + p^H X^H H^H \Phi^H\Phi H Xp + \mu \textbf{p}^Tw}
%\end{multline}


%%-------------------Algo Antonio---------------------------------------------------------
%\textbf{Algorithm}
%
%\begin{enumerate}
%	\item[] \textbf{Input} : $G = \{\mathcal{V}, E\}, L,$ sampling size $M (M=rank(L)), k = 1$
%	\item[] \textbf{Initialize} : $S = \{\}$
%	\item \textbf{while} $|S| < M$ \textbf{do}
%	\item For $S,$ compute smoothest signal $\phi_{k}^{*} \in L_{2}(S^c)$ using Proposition 2.\cite{EffSam_Aamir16}
%	\item $\nu \leftarrow \underset{\mathbf{i}}{\text{arg max}}  (\phi_{k}(i))^{2} $
%	\item Check the corresponding eigenvector that linearly independent or not? ; If yes, go to next step. If not, go to 3) and consider the second  $\underset{\mathbf{i}}{\text{arg max}}  (\phi_{k}(i))^{2} $
%	\item $S \leftarrow S\cup \nu $
%	\item \textbf{end while} 
%	\item $S_k^{opt} \leftarrow S.$
%\end{enumerate}
%%-------------------Algo Antonio---------------------------------------------------------






